Video-DCI: How Far Are VLM Agents from Human Viewers in Direct Video Corpus Interaction?

Humans answer complex visual questions by inspecting short moments, updating what they know, and redirecting attention toward missing evidence. Existing video benchmarks, however, often provide the relevant video, evaluate only final answers or isolated localization, or permit textual shortcuts, leaving multi-round visual evidence seeking underexplored. We introduce Video-DCI, a diagnostic benchmark and functionally matched human-agent protocol for Direct Video Corpus Interaction. It comprises DCI-Loc for temporal evidence localization and DCI-QA for end-to-end discovery, retention, and composition of cross-video evidence. In DCI-QA, videos within each pool are topically related, and 75% of the answers require hidden temporal evidence from multiple videos. Given only the question and video pool, humans and agents iteratively inspect bounded local windows, retain supporting evidence, and answer with cited temporal spans. Human trajectories provide reference curves for evidence acquisition and use across rounds. Experiments reveal a consistent retrieval-to-grounding gap. On DCI-Loc, frontier VLMs often retrieve and expose the reference moment, yet convert far less of this exposure into precise final citations than the human reference. On DCI-QA, the loss begins earlier and compounds across videos. Ablation studies further confirm that iterative search outperforms one-shot retrieval. Multi-round search is therefore necessary but insufficient: current agents accumulate candidates and observations more readily than precise, jointly sufficient evidence. The benchmark is available at https://huggingface.co/datasets/fireflyang/multi-video-bench-human400.

==> macros.tex <==
\RequirePackage{xspace}
\newcommand{\videodci}{Video-DCI\xspace}
\newcommand{\videodcifull}{\cmn{\textbf{D}irect Video \textbf{C}orpus \textbf{I}nteraction}\xspace}
\newcommand{\benchs}{\videodci}
\newcommand{\postskim}{post-skim evidence recovery}
\newcommand{\queryatoms}{A(q)}
\newcommand{\evidencecorpus}{\mathcal{V}}
\newcommand{\failureSet}{\mathcal{F}}
\newcommand{\indicator}{\mathbf{1}}
\newcommand{\Skim}{\mathop{\mathrm{Skim}}}
\newcommand{\Verify}{\mathop{\mathrm{Verify}}}
\newcommand{\videoOf}{\mathop{\mathrm{video}}}
\newcommand{\tIoU}{\mathop{\mathrm{tIoU}}}
\newcommand{\CRS}{\mathrm{CRS}}
% Round-1 edits: reviewed and accepted, rendered black.
% Switch back to \textcolor{blue}{#1} to re-highlight them.
\newcommand{\cm}[1]{#1}
% Round-2 edits: reviewed and accepted, rendered black.
% Switch back to \textcolor{blue}{#1} to re-highlight them.
\newcommand{\cmn}[1]{#1}
% Public release location of the benchmark (made public upon arXiv release).
% Defined with \urldef so it can be used inside footnotes and other arguments.
\urldef{\dataurl}\url{https://huggingface.co/datasets/fireflyang/multi-video-bench-human400}

